Exponential Qubit Reduction in Optimization for Financial Transaction Settlement

We extend the qubit-efficient encoding presented in [Tan et al., Quantum 5, 454 (2021)] and apply it to instances of the financial transaction settlement problem constructed from data provided by a regulated financial exchange. Our methods are directly applicable to any QUBO problem with linear inequality constraints. Our extension of previously proposed methods consists of a simplification in varying the number of qubits used to encode correlations as well as a new class of variational circuits which incorporate symmetries, thereby reducing sampling overhead, improving numerical stability and recovering the expression of the cost objective as a Hermitian observable. We also propose optimality-preserving methods to reduce variance in real-world data and substitute continuous slack variables. We benchmark our methods against standard QAOA for problems consisting of 16 transactions and obtain competitive results. Our newly proposed variational ansatz performs best overall. We demonstrate tackling problems with 128 transactions on real quantum hardware, exceeding previous results bounded by NISQ hardware by almost two orders of magnitude.

==> 01_intro.tex <==
Provable asymptotic advantages of quantum computing over classical algorithms have been shown in the \emph{fault-tolerant} regime (\cite{grover_fast_1996, shor_algorithms_1994}) and \emph{quantum computational supremacy} (\cite{harrow_quantum_2018}) has been claimed experimentally in circuit sampling tasks (\cite{arute_quantum_2019, zhong_quantum_2020, madsen_quantum_2022}).\footnote{Although some problem instances have later been shown to be classically simulable, e.g.~\cite{pan_solving_2022}.} Methods that promise to extend these computational advantages to \underline{relevant} problems with \underline{available} \emph{noisy intermediate scale quantum} (NISQ) devices have been an active field of research over the past decade. A recent breakthrough in this regard was achieved by IBM Quantum (\cite{kim_evidence_2023}), claiming evidence for the utility of said NISQ devices by simulating the evolution under an Ising Hamiltonian beyond the reach of standard\footnote{Efficient classical simulation of the experiment was claimed shortly thereafter, e.g.~using tensor networks: \cite{tindall_efficient_2023, kechedzhi_effective_2023, begusic_fast_2023}.} classical simulation methods. Most research to this end of useful NISQ algorithms is concerned with problems in Hamiltonian simulation, machine learning or energy minimization/optimization (\cite{bharti_noisy_2022, wei_nisq_nodate}). This work concerns the latter.


% \paragraph{Outline of this paper} In the introduction, we give an overview of quantum optimization in NISQ, summarize different approaches to reduce the number of qubits (\ref{subsec:quantum_optimization_intro}) and introduce the transaction settlement problem (\ref{subsec:fin_trs_settlement_intro}). We then outline our methods, including the qubit reduction (\ref{subsec:qubit_compression}), cost objective (\ref{subsec:cost}) and variational ansatz (\ref{subsec:vqa_ansatz}), before concluding with simulation (\ref{subsec:simulation_results}) and quantum hardware (\ref{subsec:hw_ionq_ibmq}) results.


\paragraph{Outline of this paper} In the introduction, we give an overview of quantum optimization in NISQ, summarize different approaches to reduce the number of qubits (\ref{subsec:quantum_optimization_intro}) and introduce the transaction settlement problem (\ref{subsec:fin_trs_settlement_intro}). We extend the qubit reduction technique introduced in ~\cite{tan_qubit-efficient_2021} to find approximate solutions to problem instances larger than previously attempted. We outline the mapping used between the quantum state and the binary variables of the problem (\ref{subsec:qubit_compression}) and how the cost can be estimated using this quantum state (\ref{subsec:cost}). We introduce a new variational ansatz derived to incorporating symmetries of the encoding scheme (\ref{subsec:vqa_ansatz}), before concluding with simulation (\ref{subsec:simulation_results}) and quantum hardware (\ref{subsec:hw_ionq_ibmq}) results.


\subsection{Quantum Optimization -- Quadratic Unconstrained Binary Optimization}\label{subsec:quantum_optimization_intro}

The optimization problem we consider in~\ref{subsec:fin_trs_settlement_intro} will generalize \emph{quadratic unconstrained binary optimization} (QUBO) problems, which have the form
\begin{equation}
    \argmin_{\myvec{x} \in \{0,1\}^I} C(\myvec x) = \argmin_{\myvec{x} \in \{0,1\}^I} \myvec x^T Q \myvec x
    \label{eq:QUBO}
\end{equation}
where $I$ is the number of binary entries of the vector $\myvec x$ and $Q$ is any real matrix, $Q \in \mathbb{R}^{I\times I}$.
Finding the vector $\myvec x$ minimizing equ.~\ref{eq:QUBO} for general $Q$ is NP hard (\cite{barahona_computational_1982}). Many combinatorial/graph problems such as MaxCut can be readily mapped to QUBO problems and a wide range of industrial applications is known. This includes training of machine learning models (\cite{date_qubo_2021}) %TODO: Read
and optimization tasks such as assignment problems (\cite{vikstal_applying_2020}), route optimization (\cite{harwood_formulating_2021}) or - the focus of this study - financial transaction settlement (\cite{braine_quantum_2019}).\footnote{For further applications see chapter 2 in \cite{punnen_quadratic_2022}.} This broad applicability and (by benchmarking existing classical solvers) \enquote{verifiable} advantage makes QUBO problems a great test-bed in the search for a useful quantum advantage. 


The solution of equation~\ref{eq:QUBO} corresponds to the ground state of an Ising Hamiltonian $H_Q$ on $I$ qubits,
\begin{equation}
    H_Q = \frac{1}{4} \sum_{i,j = 1}^IQ_{ij}(1-\sigma_z^{i})(1-\sigma_z^{j}),
    \label{eq:QUBO_hamiltonian}
\end{equation}
with $\sigma_a^i$ referring to the Pauli operator $a$ on qubit $i$. This allows mapping a QUBO problem on $I$ variables to the problem of finding the ground state of a Hamiltonian on $I$ qubits. We extend equation~\ref{eq:QUBO_hamiltonian} in section~\ref{subsec:qubit_compression} and \ref{subsec:cost} by applying the qubit compression from~\cite{tan_qubit-efficient_2021} to reduce the number of qubits to $O(\text{log}I)$ at the cost of losing the formulation~\ref{eq:QUBO_hamiltonian} as the ground state of a Hermitian operator.
\emph{Quantum solvers} (QS) to the Ising Hamiltonian or more general ground-state problems have been studied extensively. A short overview is given in table~\ref{tab:Qsolver_Annealing_QAOA_VQA_assisted} and the following: %TODO: Maybe reference some review article for further details?

\paragraph{Annealing} Introduced as early as 1994 (\cite{finnila_quantum_1994}) and inspired by simulated annealing (\cite{kirkpatrick_optimization_1984}), \emph{quantum annealing} aims to find the ground state of $H_Q$ in~\ref{eq:QUBO_hamiltonian} by \emph{adiabatically} transforming $H_{\text{tot}}(t) = s(t) H_Q + (1-s(t))H_m$, with the \emph{mixing Hamiltonian} $H_m = \sum_{j=1}^I\sigma^x_j$, over a time span $t \in [0, t_{\text{end}}]$. Here, $s(t)$ is the annealing schedule, with $s(0)=0$ and $s(t_{\text{end}})=1$. Reading out the state of the annealing device at the end of this transformation yields candidates for the optimal solution $\myvec x$. Annealing devices are not guaranteed to find optimal solutions efficiently and can only implement a limited set of Hamiltonians, often restricted in their connectivity (resulting in limitations on the non-zero entries of $Q$) (\cite{yarkoni_quantum_2022}). Despite these limitations, general purpose QUBO solvers based on hybrid classical computation and quantum annealing are commercially available with as many as 5000 (1 million) physical nodes (variables, $I$ in equ.~\ref{eq:QUBO}) for D-wave's Advantage$^\text{TM}$ annealer (\cite{inc_d-wave_nodate}).\footnote{Note that it is not public how exactly the quantum annealer is used as a subroutine in this hybrid computation.} 
\paragraph{QAOA} \emph{\textbf{Q}uantum \textbf{A}pproximate \textbf{O}ptimization \textbf{A}lgorithms}~(\cite{farhi_quantum_2014}) can be regarded as implementing a parametrized, \emph{trotterized} version of the quantum annealing schedule on gate-model based quantum computers. The parameterized $p$-layered circuit $e^{-iH_Q\beta_p}e^{-iH_m\gamma_p}...e^{-iH_Q\beta_1}e^{-iH_m\gamma_1}$ is applied to $\ket{+}^{\otimes I}$ and measured in the computational basis. This yields candidate vectors $\myvec x$ by identifying each binary variable with one qubit. The parameters $\{\beta_j, \gamma_j\}$ are classically optimized to minimize equ.~\ref{eq:QUBO} (minimize $\braket{H_Q}$). 
QAOA provides theoretical guarantees in its convergence to the exact solution for $p\to \infty$ given optimal parameters. Yet, implementing the evolution of $H_Q$ and reaching sufficient depth $p$ on NISQ devices can be infeasible in the case of many non-zero entries of $Q$.
\paragraph{Hardware efficient VQA} In this work, we make use of general \emph{Variational Quantum Algorithms} to minimize a cost estimator (in the context of quantum chemistry often referred to as VQE -- \emph{variational quantum eigensolver} (\cite{peruzzo_variational_2014}) -- and applied beyond Ising Hamiltonians). VQA's are general quantum circuit ansätze parameterized by classical parameters, hence QAOA can be seen as a special case of a VQA. We use the term \emph{hardware efficient} VQA loosely for ansätze whose gates, number of qubits and circuit depth suit current NISQ-devices. Analogously to QAOA, the parameters of the VQA circuit are optimized classically through evaluation of some classical cost function on the measured bit-vector. As we will see later, this cost function does not necessarily correspond to a Hermitian observable. 
VQAs are widely studied in the NISQ era beyond their application to combinatorial optimization problems (\cite{tilly_variational_2022, benedetti_parameterized_2019, mcclean_theory_2016}). 
Challenges, most notably vanishing gradients for expressive circuits (\cite{mcclean_barren_2018, arrasmith_effect_2021, wang_noise-induced_2021}) and remedies (\cite{liu_mitigating_2022, pesah_absence_2021, patti_entanglement_2021, grant_initialization_2019, dborin_matrix_2021, skolik_layerwise_2021, cerezo_cost_2021, schatzki_theoretical_2022, sack_avoiding_2022}) exist aplenty but will not play a central role in this paper. While the generality of VQAs allows for tailored hardware-efficient ansätze which are independent of the problem itself, this comes at the cost of losing the remaining theoretical guarantees of QAOA and adiabatic ground state computation. %TODO: We go as far as that our cost function can no longer be expressed as a hermitian observable; extensively studied, the exact form/training ... not the focus here

\paragraph{Non-VQA, quantum assisted solvers} Other quantum algorithms for solving ground-state problems have been proposed in the literature. Examples include quantum-assisted algorithms, often inspired by methods such as Krylov subspace, imaginary time evolution or quantum phase estimation. For example, quantum computers are used to calculate overlaps between quantum states employed in a classical outer optimization loop (\cite{seki_quantum_2021, kyriienko_quantum_2020, bharti_iterative_2021, takeshita_increasing_2020, motta_determining_2020, huggins_non-orthogonal_2020, stair_multireference_2020}). Although some of these approaches are variational in the circuit ansatz, they do not directly correspond to the classical-quantum feedback loop in the VQA setting described above and are beyond the focus of this work.
%TODO: More detail in thesis, e.g. see Kishor paper

\medskip


\paragraph{Classical solvers} It should be noted at this point, that approaches using classical computing for tackling QUBO problems exist. Among them\footnote{A more extensive overview can be found in chapter 11 of \cite{punnen_quadratic_2022}.} are general purpose optimization suites such as Gurobi (\cite{gurobi_optimization_llc_gurobi_2023}), CPLEX (\cite{cplex_v12_2009}) or SCIP (\cite{achterberg_scip_2009}) as well as dedicated approximation algorithms such as simulated annealing (\cite{kirkpatrick_optimization_1983}), TABU search (\cite{wang_multilevel_2012})) or the relaxation-based Goemans and Williamson (\cite{goemans_improved_1995}) algorithm which guarantees an approximation ratio of at least 0.878\footnote{Which is optimal for any polynomial time classcal algorithm assuming the unique games conjecture (\cite{khot_optimal_2005}).} for Max-Cut problems.
Due to the NP-hardness of the general problem, all classical solvers are either approximations or have no polynomial worst-case runtime guarantees.

\medskip


\paragraph{NISQ-Limitations} Quantum computers are not expected to break NP-hardness (cf. \cite{bennett_strengths_1997, aaronson_limits_2008} and the lack of any polynomial time quantum algorithm for an NP-hard problem) and it is often justified to regard quantum approaches to QUBO as heuristics \emph{hoped} to provide practical advantages rather than general purpose solvers with rigorous runtime \emph{and} optimality guarantees.
This makes benchmarking on relevant problem instances paramount in guiding the search for promising quantum algorithms. Yet, most NISQ-era quantum approaches suffer from a combination of
\begin{enumerate}
    \item \textbf{Problem size} limited by the number of available qubits
    \item Constraints on the \textbf{problem class} (connectivity of $Q$)
\end{enumerate}
making a direct application of QS to \emph{relevant} problem instances infeasible on NISQ-devices (\cite{guerreschi_qaoa_2019}). 
While 1.~is a consequence of the limited number of qubits available on NISQ devices, 2.~can be seen as a consequence of noise in the qubit and operations:
Computations become infeasible due to low coherence times and noisy gates paired with often deep circuits (e.g.~arising from the limited lattice-connectivity of devices based on superconducting qubits) upon decomposition into hardware-native gates. %QAOA - TODO: Cite
Constraints on the problem class can also arise from the fundamental design of the algorithm itself. %Annealing; Divide and Conquer, Relaxations...


How these limitations on problem size and class apply to the different QS is summarized in table~\ref{tab:Qsolver_Annealing_QAOA_VQA_assisted}. Various work has been done to address these challenges. Improved problem embeddings (\cite{date_efficiently_2019}), decomposition (\cite{mitarai_overhead_2021}), compilation and hardware-efficient ansätze are just some approaches to deal with connectivity issues. A wide variety of qubit-reduction methods has been suggested in the quantum optimization and quantum chemistry literature, see table~\ref{tab:qubit-reduction-methods}. 

Proposing a solution to the limitations in table~\ref{tab:Qsolver_Annealing_QAOA_VQA_assisted} and pushing the boundaries of QUBO problems accessible by QS is a central motivation for this work. We give a detailed description of our qubit-reduction method in section~\ref{subsec:qubit_compression}.




\input{tab_overview_compression}



\subsection{Financial Transaction Settlement}\label{subsec:fin_trs_settlement_intro}

We refer to the \emph{transaction settlement problem} as a computational task, consisting of parties $\{1,\ldots,K\}$ with balances $\{\myvec{bal}_k\}$ submitting trades $\{1,\ldots,I\}$ to a clearing house. The task faced by the clearing house is to determine the maximal set of transactions that can be executed without any party $k$ falling below its credit limit $\myvec{lim}_k$. An overview of the notation is given in table~\ref{tab:notation}, a graph representation of a transaction settlement problem with parties as nodes and transactions as edges is shown in figure~\ref{fig:TRS_settlement_example}.


\input{tab_notation-data}




In the case when not all parties have sufficient balances to meet all settlement instructions they are involved with, finding this maximal set can be difficult with classical computing resources. Intuitively, this is because a party's ability to serve outgoing transactions may depend on its incoming transactions, creating many interdependencies between different parties (cf. figure~\ref{fig:TRS_settlement_example}). 
%Practically, this can lead to challenges given high transaction volume during times of cash shortages. 
Whilst classical technology is sufficient for current transaction volumes, increases could be expected from more securities in emerging markets and digital tokens, for example. Furthermore, cash shortages make optimization more challenging as it becomes harder to allocate funds optimally among various settlement obligations, determining the priority of different trades and parties and an increased risk of settlement failures. Quantum technologies offer a potential path to mitigate these issues. 


Transactions can be conducted both in currencies and securities such as equity and bonds (hence $\myvec{bal}_k$ and $\myvec{lim}_k$ are vector-valued). 
A financial exchange may, for example, handle as many as one million trades involving 500-600 different securities by up to 100 financial institutions (parties) per day. 
% For transactions through the Central Depository (CDP) of the Singapore Exchange (SGX), the parties are around 70 financial institutions, which, representing their constituents, jointly engage in up to one million trades with 500-600 different securities per day. 









\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{img/TRS_8_example.png}
    \caption{Example of a transaction settlement problem constructed using data provided from a regulated financial exchange. Eight transactions between seven parties are depicted. Each party has initial balances for cash (\$) and different securities (S1, \ldots). The optimal solution which settles the maximal amount of transactions without violating balance constraints is indicated through \textcolor{green}{\checkmark} and \textcolor{red}{$\times$}. The solution is not unique, another optimal solution would settle T2 instead of T3. Even for a problem of only eight transactions, non-trivial dependencies between different transactions exist: For example T4 can only be settled if T5 is settled which in turn requires T8.}%maybe mention FOP, DVP
    \label{fig:TRS_settlement_example}
\end{figure}



\paragraph{QUBO formulation}

To obtain a QUBO formulation of the transaction settlement problem, we follow a slightly simplified version of \cite{braine_quantum_2019}.
% The mathematical formulation\footnote{This does not exactly correspond to the actual settlement process at SGX which makes use of dynamic \emph{cash calls} to individual parties.} 
The mathematical formulation as a binary optimization problem with inequality constraints looks as follows:
\begin{align}
    \argmax_{\myvec x}~\myvec w^T \myvec x \label{eq:max_wx}\\%~\myvec x^T A \myvec x &\\
    \textrm{subject to \emph{balance constraints}: }\sum_i x_i \myvec v_{ik} + \myvec{bal}_k - \myvec{lim}_k &\geq 0 ~\forall k \in \{1,\ldots, K\}\label{eq:constraints}
\end{align}
where for generality, a weight $w_i$ is given for each transaction $i$ and $\myvec v_{ik}$ represents the balance changes (in cash and securities) for party $k$ in transaction $i$. In practice one might choose $w_i$ proportional to the transaction value of transaction $i$, for simplicity we will always choose $w_i \equiv 1$.

The solution of this linear constrained binary optimization problem equals the solution of the mixed binary optimization (MBO)
\begin{equation}
    \argmax_{\substack{\myvec x \\ \myvec s_k \geq 0}} \left[ \myvec w^T \myvec x  - \lambda \sum_{k=1}^K \left(\sum_{i=1}^I x_i \myvec v_{ik} + \myvec{bal}_k - \myvec{lim}_k - \myvec s_k\right)^2\right]
    \label{eq:trs_qubo1}
\end{equation}
for large $\lambda$. Here, continuous slack variables $\myvec s_k \geq 0$ (element-wise) were introduced to capture the inequality constraints as penalty terms in the objective. For large enough $\lambda$, any violation of the constraints~\ref{eq:constraints} will result in a less than optimal solution vector.
Equation~\ref{eq:trs_qubo1} can directly be rewritten:
\begin{align}
    &\argmin_{\substack{\myvec x \\ \myvec s_k \geq 0}} \myvec x^T A \myvec x + \myvec b(\myvec s)^T \myvec x + c(\myvec s) \label{eq:trs_settlment_as_qubo_w_slack}\\ 
    \textrm{where: }  A &:= -\lambda V V^T,~\textrm{with }V\in \mathbb{R}^{I\times KJ}, V_{il} := (\myvec v_{ik(l)})_{j(l)} \left[\text{with }k(l) := \lceil \frac{l}{J}\rceil, j(l) := (l\text{ mod }J)+1\right]\label{eq:QUBO_trs_A}\\
    b_i(\myvec s) &:= w_i - 2\lambda \sum_{k=1}^K \left [ \myvec{bal}_k-\myvec{lim}_k-\myvec s_k \right ] \myvec v_{ik}\label{eq:QUBO_trs_b}\\
    c(\myvec s) & := - \lambda \sum_{k=1}^K \left [ \myvec{bal}_k -\myvec{lim}_k - \myvec s_k \right ]^2
\end{align}
For fixed $\myvec s$, the minimization over binary $\myvec x$ is a QUBO problem as in equ.~\ref{eq:QUBO} with $Q = A + \textrm{Diag}[\myvec b(\myvec s)]$\footnote{Here we use: $\myvec x^T \text{Diag}[\myvec b]\myvec x = \sum_{i = 1}^I b_i x_i^2 \overset{x_i^2 = x_i}{=} \myvec b^T\myvec x$}, where $\textrm{Diag}[\myvec b]$ is the matrix with the vector $\myvec b$ on the diagonal and zeros elsewhere. 








\subsection{Contribution of this work}

% We formulate the problem of settling financial transactions in a QUBO-like manner as demonstrated in~\cite{braine_quantum_2019} and find approximate solutions to settlement problems of up to 128 transactions built from data of the Singapore Exchange (SGX). 

% We present a classical preprocessing method to reduce large variances observed in the data, as well as a substitution to efficiently deal with continuous slack variables arising from constraints of the real-world problem

% Our main contribution is the generalization and extension of the exponential qubit reduction presented in~\cite{tan_qubit-efficient_2021}. We give descriptions of
% \begin{itemize}
%     \item a qubit mapping and solution sampling algorithm (section~\ref{subsec:qubit_compression}), giving a more general framework than previous work
%     \item a cost function construction allowing for simpler and more general tuning of the number of qubits used to encode correlations (section~\ref{subsec:cost})
%     \item a new circuit ansatz incorporating desirable constraints of the output state (section~\ref{subsec:vqa_ansatz})
% \end{itemize}

% We benchmark our qubit-efficient approach against standard QAOA for problems consisting of 16 transactions and obtain results slightly outperforming a direct application of QAOA. The newly proposed circuit ansatz performs best. Our exponential qubit reduction allows us to tackle problems with 128 transactions on real quantum hardware by IonQ and IBM Quantum, exceeding previous results (\cite{braine_quantum_2019}).

% To the best of our knowledge, this is the first work that tackles mixed binary optimization problems with a qubit-efficient approach on a quantum computer.


The structure of this work is as follows: In section \ref{subsec:transaction_settlement_methods}, we outline the construction of the transaction settlement instances from data provided by a regulated financial exchange. In section \ref{subsec:qubit_compression}, we use the encoding scheme listed in \cite{tan_qubit-efficient_2021} to reduce the number of qubits required and extend the ideas to include a new variational cost objective and ansatz. %, allowing for easier calculation of the gradient and sampling probabilities. 
Section \ref{subsec:simulation_results} presents the results, using the transaction settlement instances generated as a testbed for comparing our methods with QAOA and exploring different encodings. Section \ref{subsec:hw_ionq_ibmq} offers comparisons in the solutions obtained when using the exponential qubit reduction to tackle problems with 128 transactions on real quantum hardware by IonQ and IBM Quantum, exceeding previous results using quantum hardware \cite{braine_quantum_2019}. We present some analysis regarding the results obtained, before concluding with section \ref{04_Conclusion}. 
To the best of our knowledge, this is the first work that tackles mixed binary optimization problems with a qubit-efficient approach on a quantum computer.



==> 02_Methodology.tex <==

To give an overview of the methodology, we first detail how the financial settlement problem can be constructed using data provided by a regulated financial exchange (\ref{subsec:transaction_settlement_methods}). We will then describe the quantum algorithm (fig~\ref{fig:PQC_overview}) consisting of a heuristic to exponentially reduce the number of qubits (section~\ref{subsec:qubit_compression}), a cost-objective (section~\ref{subsec:cost}), a parameterized quantum circuit to generate solution bit-vectors (section~\ref{subsec:vqa_ansatz}) and finally the classical optimization (section~\ref{subsec:opt}).

\input{tikz_pqc_to_cost}


\subsection{Problem instance - Financial Transaction Settlement}\label{subsec:transaction_settlement_methods}




\paragraph{Dataset} This work uses anonymized transaction data to generate settlement problems of arbitrary size $I$.
The format of the settlement instructions made available for this purpose can be seen in table~\ref{tab:notation}. To generate a problem instance we proceeded as follows:
\begin{enumerate}
    \item Fix the number of transactions ($I$), number of parties ($K$) and an integer $R \leq I$.
    \item Choose $I-R$ random transactions from the dataset and randomly assign them to parties (sender and recipient). A single \emph{transaction} consists of a security being transferred from one party to the other and (if delivery vs payment) a cash transaction in the other direction.\footnote{To avoid confusion, we will sometimes refer to \emph{transfers} instead when only considering a single security or cash transfer.}
    \item As our dataset does not provide account balances or credit limits, we set $\myvec{lim}_k = \myvec 0$ and choose minimal non-negative balances $\myvec{bal}_k$ for each party $k$ such that all previously chosen transactions can be jointly executed without any party's balance becoming negative. The balances hence depend on the first $I-R$ transactions chosen. This choice of $\myvec{bal}_k$ is done by considering the net balance-change for each party if all transactions were conducted.
    \item Choose additional $R$ random transactions from the dataset and randomly assign them to parties (without changing the balances assigned in the previous step).
\end{enumerate}
This procedure ensures that the optimal solution contains at least $I-R$ valid transactions. Due to the minimal choice of the balances, most of the $R$ transactions chosen last are expected to be invalid in the optimal solution.







%sample graph (vgl. powerpoint to explain how generated/ maybe also use for visualization)
    % ~8 TRS
    % DVP and DOP
    % 1 security
    % Show which transactions are valid and which invalid
%mention that it is complicated to solve (in visualization sample graph)


To mitigate large differences in transaction volumes between different parties ($\text{S}\$~10-10^6$) as well as different units (cash and different securities) in the data samples, %resulting in large variances in the elements of matrix $\myvec{v}_{ij}$ in table~\ref{tab:notation}, 
we renormalize each party's balance, credit limit and transaction volume:
\begin{align}
    \forall \text{parties } k\in \{1,\ldots, K\}, \forall \text{securities } j\in \{1,\ldots, J\}: \\
    \gamma_{kj} :=& \text{mean}\left(\{|(v_{ik})_j|\}_{i=1}^I\setminus\{0\}\right)\\
    (v_{ik})_j \mapsto& \frac{(v_{ik})_j}{\gamma_{kj}}~\forall i\in \{1,\ldots, I\}\\
    (\myvec{lim}_k)_j \mapsto& \frac{(\myvec{lim}_k)_j}{\gamma_{kj}}\\
    (\myvec{bal}_k)_j \mapsto& \frac{(\myvec{bal}_k)_j}{\gamma_{kj}}
\end{align}
which, using equ~\ref{eq:max_wx} and~\ref{eq:constraints}, does not affect the optimal solution.





We show in lemma~\ref{lemma:connectivity} (appendix~\ref{app:proofs}), that the connectivity for the QUBO matrix of the transaction settlement is bounded by twice the average number of transactions per party, $\frac{4I}{K}$, plus a variance term which vanishes for d-regular graphs.

% Furthermore, for any fixed $\myvec x$, the optimal slack variables can be found by
% \begin{equation}
%     \myvec s_k(\myvec x) = \max \left(\myvec 0, -\myvec{lim}_k + \sum_{i=1}^I x_i \myvec v_{ik}+\myvec{bal}_k\right)
%     \label{eq:slack_through_x}
% \end{equation}
% where $\max(\circ, \circ)$ is to be taken element-wise. 
% Using equ.~\ref{eq:slack_through_x} removes the need for separate optimization over the slack variables. 


\subsection{Qubit-efficient Mapping}\label{subsec:qubit_compression}




\paragraph{Mapping QUBO to VQA} 
%Having shown how the transaction settlement problem can be phrased as a QUBO problem with slack variables, we now outline how to map a QUBO problem to the variational optimization of a parameterized quantum circuit (PQC) more generally than equation~\ref{eq:QUBO_hamiltonian}.
The underlying idea to solve QUBO problems with VQAs is to use the PQC to generate bit-vectors $\myvec x$. The parameters $\myvec \theta$ of the PQC are then tuned such that the generated $\myvec x$ are likely to approximately minimize equation~\ref{eq:QUBO}. 
Formally:
\begin{equation}\label{eq:QUBO_as_expectation_min}
    \min_{\myvec \theta} \mathbb{E}_{\myvec \theta}[C] := \min_{\myvec \theta} \sum_{\myvec{x} \in \{0,1\}^I} \text{Prob}_{\myvec \theta}(\myvec x) \myvec x^T Q \myvec x = \min_{\myvec \theta}\sum_{i \neq j}p_{ij}(\myvec \theta) Q_{ij} + \sum_i p_i(\myvec \theta) Q_{ii}
\end{equation}
where the right hand side only depends on the marginals $p_{ij}(\myvec \theta) := \text{Prob}_{\myvec \theta}(x_i = 1, x_j = 1)$ and $p_i(\myvec \theta) := \text{Prob}_{\myvec \theta}(x_i = 1)$. 

Instead of searching in a discrete space, this turns the problem into the optimization of the continuous parameters of a generator of bit-vectors. This appears similar but is different from relaxation-based approaches, which often replace binary variables through continuous ones to obtain a more tractable optimization problem whose solutions are projected back to a binary format: Here, the model (the PQC) directly generates bit-vectors $\myvec x$ and if it is expressive enough in the distributions $\text{Prob}_{\myvec \theta}(\myvec x)$ it parameterizes, then an optimal $\myvec \theta$ will generate an optimal bit-vector $\myvec x$ deterministically.


The steps to solve this minimization are shown in figure~\ref{fig:PQC_overview}. %We specify in later sections how we generate the bit-vectors (\ref{subsec:qubit_compression}) and how the expectation value is minimized (\ref{subsec:cost}, \ref{subsec:opt}). 
%In summary, as a generator a PQC is used, the expectation value in equation~\ref{eq:QUBO_as_expectation_min} is approximated through a cost function on finite-shot measurements of the PQC and the parameters are optimized classically.







\smallskip


The core of mapping a QUBO problem to a variational minimization problem therefore consists of specifying how to generate bit-vectors $\myvec x$ with a quantum circuit.
In standard QAOA or variational approaches this mapping is straightforward (equation~\ref{eq:QUBO_hamiltonian}): As the number of qubits $n_q$ equals the number of variables $I$, we simply measure in the computational basis (Pauli-Z) and associate the outcome 1 (-1) of qubit $q_i$ with the bit $x_i$ equal 0 (1). We use a different mapping, generalizing the qubit-efficient approach in~\cite{tan_qubit-efficient_2021}:
\paragraph{Qubit-efficient binary encoding}

We use $n_a$ qubits (\emph{ancillas}) to represent a subset of $n_a$ bits and $n_r$ qubits (\emph{register}) to provide an address labelling this subset. Compared to the approach for standard QAOA, we (partly) encode the bit-position in a binary encoded number instead of the one-hot encoded qubit-position. Hence the name \enquote{binary encoding} in table~\ref{tab:qubit-reduction-methods}.

Formally, consider a covering $\mathcal{A} = \{A_1, ..., A_{N_r}\},~N_r = 2^{n_r}$ of the set of bit-positions $B = \{1,\ldots,I\}$ with $|A_i| \in \{0, n_a\}~\forall i$ and each $A_i$ ordered. Regard the quantum state $\ket{b_1\ldots b_{n_a}}_{\text{anc}}\otimes \ket{r}_{\text{reg}}$ as corresponding to bit $A_r[l]$ (the $l^\text{th}$ entry of $A_r$) equal to $b_l~\forall l \in \{1,\ldots, n_a\}$. 
This quantum state fixes only the subset $A_r$ of the bits. In general, we interpret
\begin{itemize}
    \item Superpositions in the ancilla state $\leftrightarrow$ probabilistic sampling in the computational basis of different bit-vectors $b_1\ldots b_{n_a}$
    \item Superpositions in the register state $\leftrightarrow$ probabilistic sampling in the computational basis of different bit-sets $A_r$
\end{itemize}
resulting in the general form
%Generalizing this description, we represent a bit-vector $\myvec x$ in a quantum state of the form
\begin{equation}
    \label{eq:quantum_state_qubit_compression}
    \ket{\psi({\myvec \theta})} = \sum_{r=1}^{N_r} \beta_r(\myvec\theta) \left[a_r^{00...0}(\myvec\theta) \ket{00 ... 0}_{\text{anc}} + a_r^{00...1}(\myvec\theta) \ket{00 ... 1}_{\text{anc}} + ... \right]\otimes\ket{r}_{\text{reg}},
\end{equation}
%parameterized by $\myvec \theta$, the set of variational parameters of the PQC.
where we already indicated that the PQC parameterized by $\myvec \theta$ determines the values of the register amplitudes ($\beta_r(\myvec\theta)$) and normalized bit-vector amplitudes ($a_r^{b_1\ldots b_{n_a}}$). %A schematic explanation of this approach can be found in~\cite{tan_qubit-efficient_2021}.
We achieve an exponential compression from $n_q = I$ qubits to $n_q = n_a + \lceil\text{log}_2(I/n_a)\rceil$ in the case of a \emph{disjoint covering} (also \emph{perfect matching}). In general, a covering consisting of $|\mathcal{A}| = R$ bit-sets requires $n_a + \lceil\text{log}_2(R)\rceil$ qubits. 

For the simplest case of the \emph{minimal encoding}, defined by $n_a = 1$, each subset consists of just one binary variable with a total of $n_r = I$ subsets. A quantum state in this encoding can be written as
\begin{equation}
    \label{eq:quantum_state_min_enc}
    \ket{\psi(\myvec \theta)}_{n_a = 1} = \sum_{r=1}^{I} \beta_r(\myvec \theta) \left[a_r^0(\myvec \theta) \ket{0}_{\text{anc}} +  a_r^1(\myvec \theta) \ket{1}_{\text{anc}} \right] \otimes \ket{r}_{\text{anc}}, 
\end{equation}
and represents the bit-vector $\myvec x$ if $|a_r^i| = \delta_{ix_r}$. The total number of qubits required is $n_q = 1 + \lceil\text{log}_2(I)\rceil$.

The large decrease of qubits comes with a few drawbacks:
\begin{itemize}
    \item A single measurement in the computational basis only specifies a subset $A_r$ of the bit-positions, and it is not immediate how to sample full bit-vectors $\myvec x$.
    \item Even arbitrary state-preparation through the PQC may only allow limited distributions on the vector x. Consider for example the minimal encoding: %defined by $n_a = 1$. 
    It generates bit-vectors distributed as $\text{Prob}_{\myvec \theta}(\myvec x) = \text{Prob}_{\myvec \theta}^1(x_1)\cdot\ldots\cdot\text{Prob}_{\myvec \theta}^I(x_I) = \prod_r^{I} |a_r^{1}|^2$, where $a_r^{1}$ are the coefficients of the ancilla qubits in equation~\ref{eq:quantum_state_min_enc}, corresponding to a \emph{mean-field} approximation (\cite{veszeli_mean_2021}).
 %Every measurement only samples a single bit. Due to the independence of different measurements, any PQC and sampling procedure will generate bit-vectors distributed as $\text{Prob}_{\myvec \theta}(\myvec x) = \text{Prob}_{\myvec \theta}^1(x_1)\cdot\ldots\cdot\text{Prob}_{\myvec \theta}^I(x_I)$, corresponding to a \emph{mean-field} approximation (\cite{veszeli_mean_2021}) which we can overcome by increasing the number of ancilla qubits used.     %However, target distribution of solution vector is independent (as deterministic) 
    \item Different from QAOA, the cost objective may no longer correspond to the expectation of a Hermitian observable. This issue and a resolution are discussed in appendix~\ref{app:cost_as_observable}.
\end{itemize}


\paragraph{Sampling algorithm} 
%In summary, the proposed exponential qubit compression reinterprets the measurement in the computational basis as sampling bit-values $b_1\ldots b_{n_a}$ on subsets $A_r$ of the entries of $\myvec x$. What remains is to stitch these individual solutions together to obtain a sampling algorithm for all of $\myvec x$ (similar to the conquer step in divide and conquer approaches).

We will adopt a simple \emph{greedy} approach here, which fixes entries of $\myvec x$ as they are sampled throughout multiple measurements and concludes once every entry is sampled. We furthermore determine the covering $\mathcal{A}$ through a k-means-inspired clustering on the graph representation of the problem. %More details on this and suitable coverings $\mathcal{A}$ can be found in the appendix (\ref{app:sampling}).
Given uniform $\beta_r(\myvec \theta)$ and a disjoint covering $\mathcal{A}$, the probability of any one register not being sampled after $n_{\text{shots}}$ measurements is exponentially small, bounded by $\text{exp}(-\frac{n_{\text{shots}}}{N_r})$. %TODO: Also specify average number of samples (See Ipad, Notes Paper draft)
In practice, we sample multiple bit-vectors $\myvec x$ to find candidates for the optimal solution. This allows us to reduce the average number of measurements by reusing measurement outcomes (in particular those that were sampled multiple times before conclusion of the algorithm). Nonetheless, the qubit compression comes at the cost of significant sampling overhead.% compared to the standard encoding where each shot generates a complete bit-vector. At least $\frac{I}{n_a}$ samples are needed to generate a single bit-vectors for the qubit-efficient encoding.


%It cannot be excluded, that the PQC might prepare states with $\beta_r(\myvec \theta) \simeq 0$ in which case the sampling algorithm may never terminate. This can be avoided by choosing a suitable variational ansatz (cf.~section~\ref{subsec:vqa_ansatz}), specifying a maximal number of measurements before randomly choosing all non-sampled $\myvec x$-entries resulting in an implicit cost penalty or adding said penalty explicitly to the cost function (cf.~section~\ref{subsec:cost}).





    

     





\subsection{Cost function}\label{subsec:cost}
%TODO: For paper -> only give intuition, formulas to appendix

Having specified how to generate bit-vectors from measurement samples of the PQC fully determines $\text{Prob}_{\myvec \theta}(\myvec x)$ and hence the minimization problem in equation~\ref{eq:QUBO_as_expectation_min}. In practice, we cannot access $\text{Prob}_{\myvec \theta}(\myvec x)$ directly, but rather obtain finite-shot measurements on the state prepared by the PQC. Hence, we need to specify an estimator of the expected cost $\mathbb{E}_{\myvec \theta}[C]$. We will refer to this estimator as $\hat{C}(\myvec \theta)$.

For the explicit formulation of $\hat{C}(\myvec \theta)$, we make use of the formulation of $\mathbb{E}_{\myvec \theta}[C]$ in terms of marginal probabilities $p_{ij}(\myvec \theta) = \text{Prob}_{\myvec \theta}(x_i = 1, x_j = 1)$ and $p_i(\myvec \theta) = \text{Prob}_{\myvec \theta}(x_i = 1)$ in equation~\ref{eq:QUBO_as_expectation_min}.
For the latter we use heuristic estimators $\hat{p}_i(\myvec \theta)$ and $\hat{p}_{ij}(\myvec \theta)$ which are constructed by counting the number of times a certain bit (or pair of bits) was sampled with value equal to one. 


The exact formulas for these estimators are given in appendix~\ref{subapp:cost_estimator_formula} with a derivation for disjoint coverings in appendix~\ref{subapp:derivation_disj_covering_estimators}. Intuitively,
\begin{equation}
    \hat{p}_{ij}(\myvec \theta) 
    = (1-\hat{\mu}_{ij})\hat{q}_{ij}+\hat{\mu}_{ij}\hat{p}_i\hat{p}_j
\end{equation}
where $0\leq \hat{\mu}_{ij} \leq 1$ and the asymptotic convergence
\begin{align}
    \hat{p}_i(\myvec \theta) &\xrightarrow{n_{\text{shots}}\to \infty} \frac{\sum_{\substack{r = 1 \\ i \in A_r}}^{N_r} |\beta_r(\myvec\theta)|^2\sum_{\substack{b_k \in \{0,1\}\\b_{l_r(i)}=1}} |a_r^{b_1\ldots b_{n_a}}|^2}{\sum_{\substack{r = 1 \\ i \in A_r}}^{N_r} |\beta_r(\myvec\theta)|^2}  \label{eq:convergence_prob_est_1}\\
    \hat{q}_{ij}(\myvec \theta)&\xrightarrow{n_{\text{shots}}\to \infty} \frac{\sum_{\substack{r = 1 \\ i,j \in A_r}}^{N_r} |\beta_r(\myvec\theta)|^2\sum_{\substack{b_k \in \{0,1\}\\b_{l_r(i)}=b_{l_r(j)}=1}} |a_r^{b_1\ldots b_{n_a}}|^2}{\sum_{\substack{r = 1 \\ i,j \in A_r}}^{N_r} |\beta_r(\myvec\theta)|^2} \label{eq:convergence_prob_est_2}
\end{align}
motivates the expressions $\hat{p}_i$ and $\hat{p}_{ij}$.

Following equation~\ref{eq:QUBO_as_expectation_min}, the cost estimator $\hat{C}(\myvec \theta)$ for the transaction settlement problem then takes the form 

\begin{equation}
    \hat{C}(\myvec \theta) = \sum_{\substack{i,j = 1\\i\neq j}}^I \hat{p}_{ij}(\myvec \theta) A_{ij} + \sum_{i = 1}^I \hat{p}_{i}(\myvec \theta) (A_{ii}+b_i(\myvec s)) + c(\myvec s)
    \label{eq:cost_estimator}
\end{equation}

which is optimized with respect to $\myvec \theta$ and the slack variables $\myvec s = (\myvec s_1, \ldots, \myvec s_K) \geq 0$. 
The optimal slack variables can be obtained straightforwardly using 
\begin{equation}
    \hat{\myvec s}_k(\myvec \theta) = \max \left(\myvec 0, -\myvec{lim}_k + \sum_{i=1}^I \hat{p}_i(\myvec \theta) \myvec v_{ik}+\myvec{bal}_k\right)
    \label{eq:slack_estimator}
\end{equation}
where $\max(\circ, \circ)$ is to be taken element-wise. 
The optimal slack variables substitute $\myvec s$ in equ~\ref{eq:cost_estimator}, thus removing the need for separate optimization over the slack variables. 
% We have not written the dependence of $\hat{C}$ on the slack variables explicitly, as instead of optimizing them separately we substitute $\myvec s$ by
% \begin{equation}
%     \hat{\myvec s}_k(\myvec \theta) = \max \left(\myvec 0, -\myvec{lim}_k + \sum_{i=1}^I \hat{p}_i(\myvec \theta) \myvec v_{ik}+\myvec{bal}_k\right)
%     \label{eq:slack_estimator}
% \end{equation}
% in equation~\ref{eq:cost_estimator} (cf.~\ref{eq:slack_through_x}).



\paragraph{Remarks:} 
\begin{enumerate}
    \item It is not possible to express equation~\ref{eq:cost_estimator} as the expectation of a Hermitian observable on a state of the form of equation~\ref{eq:quantum_state_qubit_compression} due to denominators in the expressions for $\hat{p}$, $\hat{q}$ (equ.~\ref{eq:p_hat_pauli}, \ref{eq:q_hat_pauli} in appendix) and $\hat{\mu}_{ij}$ (equ.~\ref{eq:estimator_mu}) as well as the functional form of $\hat{\myvec s}$. We will show in appendix~\ref{app:cost_as_observable} how this problem can be resolved for fixed $\myvec s$ given uniform $\beta_r(\myvec \theta)$.
    %\item The choice of the marginal probabilities $\hat{p}_i$ and $\hat{p}_{ij}$ is intuitive due to equation~\ref{eq:convergence_prob_est_1} and \ref{eq:convergence_prob_est_2}. However, their correspondence to the actual probabilities obtained from the sampling algorithm described in the previous section is not clear. While their estimation of these probabilities is unclear for general coverings $\mathcal{A}$, we give a proof for disjoint coverings $\mathcal{A}$ in appendix~\ref{app:marg_prob_from_sampling}.
    \item In the limit of the \emph{full encoding} ($n_a = I$, $n_r = 0$), we get \[\hat{p}_{ij} = \hat{q}_{ij} = \left \langle \mathds{1}_{\min\{i,j\}-1}\otimes\ket{1}\bra{1}\otimes\mathds{1}_{|i-j|-1}\otimes\ket{1}\bra{1}\otimes \mathds{1}_{I-i-j}  \right \rangle_{\mathcal{M}} \]
    and
    \[\hat{p}_i = \left \langle \mathds{1}_{i-1}\otimes\ket{1}\bra{1}\otimes \mathds{1}_{I-i}  \right \rangle_{\mathcal{M}}\]
    resulting in the \enquote{standard} cost estimator identical to e.g.~QAOA.
    \item Runtime and memory cost: 
    %The cost estimator $\Hat{C}(\myvec \theta)$ is a function of $O(I^2)$ sums over the set of measurement outcomes in the computational basis. The naive run-time for classically computing the cost estimator hence scales as $O(n_{\text{shots}}I^2)$, while the memory required only scales as $O(n_{\text{shots}}+I^2)$. Our approach does not require full tomography with memory requirements as high as $O(4^I)$. In the most straightforward estimation, only single-qubit Pauli-Z measurements are required. In further extensions, methods such as classical shadows (\cite{huang_predicting_2020}) may be used to more efficiently estimate the cost and reduce $n_{\text{shots}}$.
    The naive run-time for classically computing the cost estimator scales as $O(n_{\text{shots}}I^2)$, while the memory required only scales as $O(n_{\text{shots}}+I^2)$. Our approach does not require full tomography with memory requirements as high as $O(4^I)$. %In the most straightforward estimation, only single-qubit Pauli-Z measurements are required. 
    In further extensions, methods such as classical shadows (\cite{huang_predicting_2020}) may be used to more efficiently estimate the cost and reduce $n_{\text{shots}}$.
\end{enumerate}



If certain registers are hardly sampled, i.e. $ |\beta_r(\myvec\theta)|^2\simeq 0$, we may encounter division by zero in the expressions for $\hat{p}_i$ and $\hat{q}_{ij}$. In practice, this can be dealt with by setting the corresponding estimators to $1/2$ whenever estimates for $|\beta_r(\myvec\theta)|^2$ fall below some $\epsilon > 0$, resulting in indirect penalization. Alternatively, we can add an explicit regularization term $\hat{R}(\myvec \theta) = \eta \sum_{r = 1}^{N_r}\left [\hat{r}_r(\myvec \theta) -\frac{1}{N_r} \right]^2$ to the cost function. %This is detailed in appendix~\ref{subapp:cost_regularization} and the gradient of the cost estimator is given in appendix~\ref{subapp:gradient_cost}.

%\paragraph{Regularization term for uniform register sampling} If certain registers are hardly sampled, i.e. $\langle \mathds{1}_{n_a} \otimes \ket{r}\bra{r} \rangle_{\mathcal{M}} \simeq 0$ we may encounter division by zero in the expressions for $\hat{p}_i$ and $\hat{q}_{ij}$. In practice, this can be dealt with by setting the corresponding estimators to $1/2$ (or any other value) when $\langle \mathds{1}_{n_a} \otimes \ket{r}\bra{r} \rangle_{\mathcal{M}} < \epsilon$ for some $\epsilon > 0$. In the optimization of $\myvec \theta$, such states will be penalized as they inflate the value of $\hat{C}(\myvec \theta)$. Alternatively, this penalization can be made explicit by adding a term
%\begin{align}
%    \hat{R}(\myvec \theta) &= \eta \sum_{r = 1}^{N_r}\left [\hat{r}_r(\myvec \theta) -\frac{1}{N_r} \right]^2 \label{eq:reg_pres_penalty}\\
%    \text{with:   } \hat{r}_r(\myvec \theta) &=\langle \mathds{1}_{n_a} \otimes \ket{r}\bra{r}\rangle_{\mathcal{M}}.
%\end{align}


%\paragraph{Gradients of the cost function} When optimizing $\hat{C}(\myvec \theta)$ with respect to $\myvec \theta$ we may want to make use of the gradient $\nabla_{\mthet}\hat{C}$. For this, note that both terms in the quotient for $\hat{p}_i$ and $\hat{q}_{ij}$ are given as linear combinations of Pauli-expectation values (equation~\ref{eq:p_hat_pauli} and \ref{eq:q_hat_pauli}). For many variational ansätze - in particular those consisting of single-qubit Pauli-rotations used in this paper - this allows to easily calculate gradients $\nabla_{\mthet}[\hat{p}_i]$ and $\nabla_{\mthet}[\hat{q_{ij}}]$ through the parameter-shift rule (\cite{mitarai_quantum_2018, schuld_evaluating_2019}). Similarly, the gradients of $\hat{\mu}_{ij}$ and $\hat{r}_r$ can be calculated by applying the parameter-shift rule.
%Through application of the chain-rule, the gradient of $\hat{C}\left(\{\hat{p}_i\}_i, \{\hat{q}_{ij}\}_{ij}, \{\hat{\mu}_{ij}\}_{ij};\{\hat{r}_r\}_{r}\right )$ is obtained, the explicit form of which is given in appendix~\ref{subapp:gradient_cost}.






%TODO: Make connection to Ben's paper and the way the cost is calculated there



\subsection{Variational ansatz}\label{subsec:vqa_ansatz}

In this work we consider two types of PQC:
\begin{itemize}
    \item A \emph{hardware-efficient} ansatz consisting of RY rotations and entangling CNOT layers.
    \item A \emph{register-preserving} ansatz of conditional RY rotations incorporating constraints and symmetries tailored to the qubit-efficient encoding.
\end{itemize}
Both variational circuits are depicted in figure~\ref{fig:var_ansatz}. The hardware-efficient ansatz was used identically in~\cite{tan_qubit-efficient_2021}, the register-preserving ansatz is one of the main contributions of this work.



We mentioned difficulties arising from vanishing register-amplitudes in the previous section. We will now formally define register-uniform quantum states and register-preserving circuits before discussing the advantages offered by them:


% Definition register-uniform
\begin{restatable}[Register-uniform]{de}{definitionreguniform}
    \label{def:reg_uniform}
    We call a quantum state $\ket{\psi}_{ar}\in \mathcal{H}_{\text{anc}}\otimes\mathcal{H}_{\text{reg}}$ \emph{register-uniform} with respect to the orthonormal basis $\left(\ket{1},\ldots ,\ket{N_r}\right)$ of $\mathcal{H}_{\text{reg}}$, if it can be written as
    \begin{equation}
        \ket{\psi} = \frac{1}{\sqrt{N_r}}\sum_{r = 1}^{N_r}\ket{\phi_r}_{\text{anc}}\otimes\ket{r}_{\text{reg}}
        \label{eq:reguniform_def}
    \end{equation}
    where $\ket{\phi_r}_{\text{anc}} \in \mathcal{H}_{\text{anc}}$ is arbitrary with $\braket{\phi_r | \phi_r}_{\text{anc}} = 1 ~\forall r$. 
\end{restatable}



% Definition register-preserving
\begin{restatable}[Register-preserving]{de}{definitionregpreserving}
    \label{def:reg_preserving}
    We call a unitary $U$ acting on $\mathcal{H}_{\text{anc}}\otimes\mathcal{H}_{\text{reg}}$ \emph{register-preserving} with respect to the orthonormal basis $\left(\ket{1},\ldots ,\ket{N_r}\right)$ of $\mathcal{H}_{\text{reg}}$ if it always maps register-uniform states to register-uniform states (with respect to the same basis).
\end{restatable}
%TODO: Maybe mention that register-preserving could also be defined more generally (not just for uniform registers...)
The set of register-preserving unitaries with respect to the same basis is closed under concatenation. 
Our register-preserving ansatz first prepares the register-uniform plus state $\ket{+}^{\otimes n_q} = H^{\otimes n_q} \ket{0}$ ($H$ being the Hadamard gate) and then acts through register-preserving unitaries on it.

\paragraph{Notation} We use the bra-/ket-notation only for normalized states. Furthermore, Latin letters inside bra and ket indicate computational basis states, while Greek letters indicate general quantum states.
We will refer to \emph{register-preserving circuits} as quantum circuits which output register-uniform states with respect to the computational basis (and fix said basis from now on, omitting further mention of it). 




The following claims about register-uniform states and register-preserving circuits are proved in appendix~\ref{app:proofs}:

% Equivalent definitions of register-uniform
\begin{restatable}[]{lm}{lemmareguniform}
    \label{lemma:reg_uniform}
    The following is equivalent to a state $\ket{\psi}\in \mathcal{H}_{\text{anc}}\otimes\mathcal{H}_{\text{reg}}$ being register-uniform:
    \begin{equation}
        \bra{r}\text{tr}_{\mathcal{H}_{\text{anc}}}(\ket{\psi}\bra{\psi})\ket{r} = \frac{1}{N_r} ~\forall r\in \{1,\ldots, N_r\}
        \label{eq:reguniform_equivalent_def}
    \end{equation}
\end{restatable}



% Equivalent definitions of register-preserving
\begin{restatable}[]{thm}{theoremregpreserving}
    \label{theorem:reg_preserving}
    The following are equivalent for a unitary $U$ acting on $\mathcal{H}_{\text{anc}}\otimes\mathcal{H}_{\text{reg}}$:
    \begin{enumerate}[label=(\roman*)]
        \item $U$ is register-preserving
        \item $U (\ket{\phi}_{\text{anc}}\otimes\ket{r}_{\text{reg}}) = (U_r\ket{\phi}_{\text{anc}})\otimes\ket{f(r)}$ where $U_r$ is a unitary on $\mathcal{H}_{\text{anc}}$ $\forall r$ and $f: \{1,\ldots,N_r\}\to\{1,\ldots,N_r\}$ is bijective.
        \item $U$ can be written as a sequence of unitary matrices on $\mathcal{H}_{\text{anc}}$ conditioned on a subset of register-qubits and basis-permutations on the register.
    \end{enumerate}
\end{restatable}
Note\footnote{To avoid confusion with the \emph{permutation operator} used in quantum physics which refers to permuting particle-labels.}, that in theorem~\ref{theorem:reg_preserving} we refer to \emph{basis}-permutations, not \emph{qubit}-permutations, although former contains the latter.



\input{tikz_ansatz}


Theorem~\ref{theorem:reg_preserving} provides a list of ingredients that may be used to construct register-preserving variational ansätze. Namely, we can combine conditional unitaries (such as CNOT, Toffoli gates), acting on the ancillas and conditioned on the register-qubits, with arbitrary unitaries that only act on the ancilla qubits. Furthermore, we can permute computational basis states on the register qubits. These permutations could be cryptographic permutation pads~\cite{kuang_quantum_2022}, binary adder circuits~\cite{draper_addition_2000} or heuristic constructions from NISQ-friendly gates such as CNOT, SWAP and X gates.

When defining register-preserving circuits, we demand that \emph{any} register-uniform state is mapped to a register-uniform state. This may not always be necessary. In the case of this work, we always start with the same input state $\ket{+}^{\otimes n_q}$ which allows more general unitaries than theorem~\ref{theorem:reg_preserving}, as the following lemma demonstrates:

\begin{restatable}[]{lm}{lemmaregpreservingsometimes}
    \label{lemma:reg_pres_sometimes}
    For register-uniform states as in equation~\ref{eq:reguniform_def} with $\braket{\phi_{r_1}|\phi_{r_2}}_{\text{anc}}\in \mathbb{R}~\forall r_1, r_2\in \{1,\ldots, N_r\}$, a unitary $U = \mathds{1}_{\text{anc}}\otimes U_\text{reg}$ only non-trivially acting on the register-qubits always maps $\ket{\psi}$ to a register-uniform state if and only if
    \begin{equation}
        (U^\dagger)_{r_1s}U_{sr_2} \in i\mathbb{R}~ \forall r_1,r_2,s\in \{1,\ldots, N_r\} \text{ with } r_1<r_2.
    \end{equation}
\end{restatable}
While theorem~\ref{theorem:reg_preserving} only allows permutations on the register-qubits, this lemma allows (a single) application of $\text{exp}\left(-i\frac{\theta}{2}P\right)$ for any self-inverse permutation $P$, e.g. R$X^n$ rotations or the RBS gate, on the register-qubits.
The condition $\braket{\phi_{r_1}|\phi_{r_2}}_{\text{anc}}\in \mathbb{R}$ is trivially fulfilled for states which are a real-valued linear combination of computational basis states such as $\ket{+}^{\otimes n_q}$.

%\smallskip


\paragraph{Our ansatz} The circuits used in this work are shown in figure~\ref{fig:var_ansatz}. The register-preserving circuit acts with conditional RY rotations on every ancilla-qubit, conditioned on individual register-qubits. The RY rotation on ancilla-qubit $b$ conditioned on register-qubit $c$ can be regarded as a parameterized rotation on $b$ for half the registers (those registers $r$, for which the binary encoding of r has a 1 at position $c$). A basis permutation layer consisting of CNOTs is added to assure consecutive conditional RY rotations act on a different set of registers (this basis permutation layer is omitted if only a single layer is used, $d=1$).


In terms of optimization parameters, we optimize $n_a*n_r$ parameters per register-preserving layer and $n_q = n_r+n_a$ for the hardware-efficient ansatz. 




\paragraph{Discussion register-preserving ansatz}
Only allowing register-preserving gates in the variational ansatz imposes challenges in keeping the variational ansatz both expressive and NISQ-friendly, at least on superconducting hardware (cf. section~\ref{subsec:hw_ionq_ibmq}). On the other hand, we see the following motivations and advantages for exploring register-preserving circuits:
\begin{enumerate}
    \item Respect the symmetries of the qubit-efficient approach: 
    % It is not clear what, if anything, can be gained by varying over non-uniform register-probabilities in the estimator of the cost function in section~\ref{subsec:cost}. 
    In light of challenges associated to barren plateaus for over-expressive ansätze, incorporating symmetries into the circuit architecture - here: register-preservation and real-valued amplitudes\footnote{Real-valued amplitudes are the reason we only make use of RY rotations (instead of RX, RZ).} in the computational basis - is promising as it has been shown to help with the problem of vanishing gradients (\cite{schatzki_theoretical_2022, liu_variational_2019}).
    \item Numeric stability: The cost estimator $\Hat{C}(\myvec \theta)$ (equ.~\ref{eq:cost_estimator}) makes use of estimators for the register-amplitudes $|\beta(\myvec \theta)|^2$. These can be fixed to $\frac{1}{N_r}$ for a register-preserving circuits, adding numerical stability (especially as the terms affected are in the denominator) and reducing the computational overhead. In figure~\ref{fig:shot_noise_variance_grad}, we visualize the variance of the gradient-estimator with respect to shot noise at fixed parameters $\myvec \theta$. The register-preserving ansatz shows much smaller variance, which suggest a lower number of required shots $n_{\text{shots}}$ (cf.~bullet 3.). %Especially for small circuit depths, the gradient is much less sample-dependent than in the case of the hardware-efficient ansatz. This may allow similar estimation quality with fewer shots. 
    \item Sampling overhead: Register-uniform states minimize the expected number of samples needed to cover each register (\cite{boneh_coupon-collector_1989}).  %page 18
    Furthermore, theorem~\ref{theorem:reg_preserving} $(ii)$ shows, that the net effect of any register-preserving unitary on the register-qubits is a permutation. If this permutation $P: \ket{r}\mapsto \ket{f(r)}$ is easily inverted, then the bit-vector sampling can be made deterministic in the register (without otherwise impacting the prediction), by using the input state $H^{\otimes n_a}\ket{0}_{\text{anc}}\otimes P^{-1} \ket{r}_{\text{reg}}$ instead of $H^{\otimes n_a+n_r}\ket{0}$. In any case, we can reduce the number of circuit evaluations needed by using initial states of the form $H^{\otimes n_a}\ket{0}_{\text{anc}}\otimes \ket{r}_{\text{reg}}$ and ensuring that we sample a different register $f(r)$ in every run by iterating over $r \in \{1,\ldots, N_r\}$. 
    \item Expression as expectation value of Hermitian observable: As all denominators in the expressions for $\hat{p}_i$, $\hat{q}_{ij}$ and all of $\hat{\mu}$ are replaced by constants, this allows -- for fixed $\myvec s$ -- to express $\hat{C}(\myvec \theta)$ as the expectation value of a Hermitian observable (although the product $\hat{p}_i \hat{p}_j$ requires preparation of a product state, see appendix~\ref{app:cost_as_observable}).
    A majority of the literature (including aforementioned classical shadows) and software are tailored primarily for Hermitian expectation values. 
    Areas include theoretical results (e.g.~adiabatic theorem), the variational ansatz and optimizer itself, estimation and error mitigation as well as fault-tolerant methods for the evaluation of expectation values.
    Expressing our cost function as a Hermitian expectation hence widens the cross-applicability of other results and code-bases.
    %This allows to apply existing results on the minimization of Hermitian expectation values (more details in appendix~\ref{app:cost_as_observable}).
\end{enumerate}


\begin{figure}
    \captionsetup{width = 0.5\linewidth}
    \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=0.5\linewidth}}]{figure}%[\FBwidth]
    {\caption[Shot-noise gradient]{\colorbox{lightgray!30!white}{16 Transactions, 12 parties, 6 qubits, $n_a = 4$} | Variance in partial derivatives of cost estimator over ten samples ($10^4$ shots each). The variance was in turn averaged over all entries of the gradient. This was done for circuits of different depth (x-axis), for each of which we uniformly sampled 25 different parameters $\myvec \theta$ (scatter). The median over the different parameters is depicted as a solid line, the inter-quartile range as a shaded region.}\label{fig:shot_noise_variance_grad}}
    {\includegraphics[width=1\linewidth]{img/Gradient-variance-SP104_depth1-12_n_a4_10kshots.png}}
\end{figure}





\subsection{Optimization}\label{subsec:opt}

Many different optimization procedures have been suggested in the literature to find the optimal parameters for a PQC through classical optimization. This includes the parameter-initialization (\cite{truger_warm-starting_2023, egger_warm-starting_2021, akshay_parameter_2021, grant_initialization_2019, mitarai_generalization_2019}), choice of meta-parameters (\cite{goh_techniques_2022}) as well as the parameter update itself (\cite{barkoutsos_improving_2020, schuld_evaluating_2019, ostaszewski_structure_2021, nakanishi_sequential_2020, skolik_layerwise_2021}, an overview of gradient-based and gradient-free optimizers can be found in section D. of \cite{bharti_noisy_2022}). 
%Furthermore, a variety of techniques has been proposed to deal with challenges such as vanishing gradients (\cite{liu_mitigating_2022, pesah_absence_2021, patti_entanglement_2021, grant_initialization_2019, dborin_matrix_2021, skolik_layerwise_2021, cerezo_cost_2021}).

While the optimization of a PQC has been shown to be NP-hard (\cite{bittel_training_2021}) and may well be the most important ingredient to practical advantage for any quantum QUBO solver, the focus of this work is on the qubit-efficient methods rather than on the optimization itself. Our results were obtained with two different commonly used optimizers: The gradient-free optimizer COBYLA (implemented in scipy~\cite{virtanen_scipy_2020}) as well as standard gradient descent, with gradients calculated through the parameter-shift rule (\cite{mitarai_quantum_2018, schuld_evaluating_2019}). 

The full optimization step for updating the circuit parameters $\myvec \theta^{(n)}\mapsto \myvec \theta^{(n+1)}$ is depicted in figure~\ref{fig:PQC_overview}.




==> 03a_simulation_results.tex <==

% Repeat of subsection title and intro text of section3
% In this section we present and discuss the simulated results on transaction settlement problems with 16 transaction instructions. We restrict the number of transactions to compare our qubit-efficient methods with simulated QAOA, the latter requiring as many qubits as variables.
% In the next section we will present simulation and hardware results for up to 128 transactions.

% Figure~\ref{fig:training_trace_16TRS} shows the training convergence for one configuration averaged over different uniformly random chosen initial parameters of the PQC. While the COBYLA optimizer returns optimized parameters after only a few hundred or even less steps, it often does not converge to a cost as low as gradient descent (DESC). % reliably does for the hardware-efficient and register-preserving ansatz. 
% Here, the Register-preserving ansatz appears to converge to better solutions compared to the hardware-efficient PQC. Deeper circuits yield lower cost values for the qubit-efficient approaches, while no significant differences are observed for QAOA between depth (QAOA p-value) $1-10$ besides more steps to convergence for larger depth.
% We note that QAOA was trained by alternating the optimization of the slack parameters and the circuit parameters (50 alternations with a maximum of 1000 steps for the COBYLA optimization of the circuit in each step). This is due to the variational ansatz which depends on the QUBO matrix and hence on the slack variables (cf. equation~\ref{eq:trs_settlment_as_qubo_w_slack}), rendering the substitution~\ref{eq:slack_estimator} infeasible (however, it can still be used in the slack variable adjustment after each optimization of the PQC parameters). This interdependence between the ansatz and the slack variables results in more training steps and spikes of the training cost whenever the slack variables are adjusted. It furthermore means that quantitative cost values are not directly comparable to our qubit-efficient approach.


\paragraph{Training convergence} Figure~\ref{fig:training_trace_16TRS} shows the training convergence for one problem configuration averaged over different random initial parameters of the PQC. While COBYLA returned optimized parameters within a few hundred steps or less, its cost value is consistently outperformed by gradient descent (DESC), especially for increasing number of circuit parameters.

The register-preserving ansatz not only outperforms the hardware efficient PQC, but also produces solutions with tighter spread. For all the qubit-efficient approaches, deeper circuits also improved the performance.

For QAOA, the substitution in equ~\ref{eq:slack_estimator} to optimize both slack variables and variational parameters simultaneously is infeasible as the variational ansatz depends on the QUBO matrix and by extension, the slack variables (cf. equation~\ref{eq:trs_settlment_as_qubo_w_slack}). Results for QAOA were obtained by alternating the optimization of slack variables and circuit parameters 50 times, with up to $10^3$ COBYLA-iterations to update the circuit parameters at each cycle. The optimization landscape appears to be dominated by the slack variables, and each update changes the optimization landscape for the variational parameters. This unusual optimization landscape is likely the reason why no significant improvements were observed for increasing p-values.

From our brief comparison, hardware efficient ansätze appear to be more suited for MBO problems as they are agnostic to changes in the QUBO matrix. Despite these challenges, we maintain our QAOA results for the purposes of comparison, and leave the exploration of more effective implementations of the QAOA to MBO to future work.



\begin{figure}
    \centering
    \includegraphics[width = 1.0\linewidth]{img/FGRID_SPSP87_16T_n_shots20k_n_a1_shade.png}
    \caption[Training traces]{\colorbox{lightgray!30!white}{16 Transactions, 10 parties, 5 (register-efficient) / 16 (QAOA) qubits, $n_a = 1$, $2\times 10^4$ shots} | Training traces for different circuit ansätze (title) applied to a transaction settlement problem with 16 transactions. Two different optimizers, COBYLA (gradient-free) and gradient descent (DESC) were used in the qubit-efficient approach while only COBYLA was used for QAOA. The depth of the circuit (in number of layers / p-value for QAOA) is given in square brackets. The solid lines depict means over 25 (qubit-efficient) and 10 (QAOA) different training runs with random starting points. The 95\% confidence interval is given as a shaded region. Quantitative values against QAOA are not comparable due to different cost-objectives.} %https://seaborn.pydata.org/tutorial/error_bars.html#confidence-interval-error-bars
    \label{fig:training_trace_16TRS}
\end{figure}

% \FloatBarrier


\paragraph{Bit-vector quality} As the cost estimator used in the optimization is only a proxy for the actual quality of the bit-vectors $\myvec x$ generated, we show the empirical cumulative distribution of the cost associated to bit-vectors generated from the trained PQC in figure~\ref{fig:cdf}. We normalized the cost for each transaction settlement problem and averaged over different configurations (three settlement problems, $n_a \in \{1,4,8\}$ for~\ref{fig:cdf_QAOA}, COBYLA and gradient descent, up to 25 training runs), drawing 50 bit-vectors per configuration.

Subfigure~\ref{fig:cdf_QAOA} shows the cumulative distributions for both the qubit-efficient approach and QAOA.  Except for the hardware-efficient ansatz with one layer, our qubit-efficient approach performs better than QAOA on average. As in the training traces, no significant differences in the results for QAOA were found by varying the depth (p-value) from one to ten. The register-preserving ansatz performs best over all depths.

In subfigure~\ref{fig:cdf_AncReg}, weak improvement can be observed by using 8 instead of 1 ancilla qubits and by adding another register-qubit ($n_r+ =1$). 

% All approaches perform better than the random sampling of bit-vectors. 
During the training, we observed that gradient descent yields better minima than COBYLA in the cost estimator but tends to \emph{sparse} solutions, i.e. the associated distribution on bit-vectors is strongly concentrated around a single value (cf. figure~\ref{fig:cdf_HW}). Here, redundant encoding of bit-vector-positions in the ancillas (i.e.~$n_r+ > 0$) was found to help in generating more diverse solution candidates.



\begin{figure}
    \centering
    \begin{subfigure}[t]{0.52\textwidth}
        \includegraphics[width =1.0\linewidth]{img/cdf-plot_Sampler_QAOA_n_a1-8_shots10k.png}
        \caption{Different circuit ansätze (hardware-efficient, register-preserving and QAOA) are compared at different depths (number of layers / p-value). $n_a, n_r+ \in \{(1,0),(4,0),(8,0),(8,1)\}$, COBYLA.}
        \label{fig:cdf_QAOA}
    \end{subfigure}
    \begin{subfigure}[t]{0.47\textwidth}
        \includegraphics[width =1.0\linewidth]{img/cdf-plot_AncReg-noQAOA_n_a1-8_shots10k.png}
        \caption{Different encodings with one and eight (both as a disjoint covering, $n_r+ = 0$, and as a redundant covering, $n_r+ = 1$) ancilla qubits are compared for different optimization algorithms. Both COBYLA and gradient descent are included.}
        \label{fig:cdf_AncReg}
    \end{subfigure}
    \caption[Empirical cumulative distribution function]{\colorbox{lightgray!30!white}{16 Transactions, 10-13 parties, 5-16 qubits, $10^4$ shots} | Empirical cumulative distribution function of normalized cost (with zero corresponding to the cost of the optimal bit vector) over bit-vectors generated by different trained PQCs: For a given cost x, the empirical probability y of generating bit-vectors with cost at most x is plotted. Insets show the area with the lowest 5\% of the cost. In the calculation of the cost, equation~\ref{eq:trs_settlment_as_qubo_w_slack} was used with optimal slack-variables $\myvec s (\myvec x)$ for a given bit-vector $\myvec x$. The distribution for uniformly random bit-vectors is shown as a grey dotted line.}
    \label{fig:cdf}
\end{figure}

==> 03b_hardware_results.tex <==
To investigate the generation of bit-vectors on real quantum hardware (QPU), we optimized different configurations of both register-preserving and hardware-efficient PQCs on a simulator for 16 and 128 transactions. The pre-trained circuit parameters were then executed on the Geneva/Hanoi QPU provided by IBM Quantum and the Harmony/Aria QPU provided by IonQ.\footnote{Different backends from both providers were used as \texttt{ibmq\_geneva} was retired while this work was in process and \texttt{ionq\_harmony} only provides 11 qubits, necessitating the larger \texttt{ionq\_aria} device for 128 transactions with 16 ancillas.}
The resulting cost-distributions of generated bit-vectors for a settlement problem with 16 transactions and 10 parties / 128 transactions and 41 parties are depicted in figure~\ref{fig:cdf_HW} and \ref{fig:ionq_ibm_128trs_HW}.


% To investigate the generation of bit-vectors on real quantum hardware (QPU), we executed different configurations of both register-preserving and hardware-efficient PQCs on a simulator for 16 and 128 transactions. The circuit parameters were pre-trained on a noise-free simulator, potentially resulting in systematic errors (relative to a run-time optimization on the noisy device itself) when executed on hardware. %TODO: Citation?
% The optimized circuit parameters were then executed on the Geneva/Hanoi QPU provided by IBM Quantum and the Harmony/Aria QPU provided by IonQ.\footnote{Different backends from both providers were used as \texttt{ibmq\_geneva} was retired while this work was in process and \texttt{ionq\_harmony} only provides 11 qubits, necessitating the larger \texttt{ionq\_aria} device for 128 transactions with 16 ancillas.} %TODO: Link to QPU / cite properly


% The transaction settlement problem with 128 transactions (visualized in the appendix, figure~\ref{fig:graph_settlement_instructions_128}) has up to 22 transfers per party, still far from the real-world scenario outlined in section~\ref{subsec:transaction_settlement_methods} but significantly more complex than the toy example in figure~\ref{fig:TRS_settlement_example}.


% The resulting cost-distributions of generated bit-vectors for a settlement problem with 16 transactions and 10 parties / 128 transactions and 41 parties is depicted in figure~\ref{fig:cdf_HW} and \ref{fig:ionq_ibm_128trs_HW}.



\paragraph{IBMQ vs IonQ} For $4$ layers of the register-preserving circuit (\ref{fig:cdf_reg-pres-HW}), the IBMQ results are significantly worse than for IonQ. This can partly be attributed to the connectivity requirements of the long-range conditional Y-Rotations used in the register-preserving ansatz (figure~\ref{fig:reg-pres_ansatz}). This favours the all-to-all connectivity of \texttt{ionq\_harmony}, which foregoes the need for depth-increasing SWAP networks. The hardware-efficient ansatz (\ref{fig:cdf_hwe-HW}) on the other hand is compatible with the lattice connectivity of IBMQ devices and shows similar performance for both QPUs. 

%When compiled to IBMQ hardware, the gate-count scales almost linearly in $n_a*n_r$ for the register-preserving circuit and in $n_q = n_a+n_r$ for the hardware-efficient ansatz, explaining the unfavourable performance of the register-preserving ansatz on \texttt{ibm\_geneva}. 
%While the compilation on IonQ devices is proprietary, the all-to-all connectivity in the trapped ion's system forgoes the need for SWAP networks when implementing the conditional RY rotations, which should result in a lower overall gate-count.



For 128 transactions, the benchmarked IonQ device (\texttt{ionq\_aria}) slightly outperforms IBMQ (\texttt{ibm\_hanoi}) even with the hardware-efficient ansatz, the results of which are depicted in figure~\ref{fig:ionq_ibm_128trs_HW}.



% \FloatBarrier

\paragraph{Impact of noise}
In general, the noisy results obtained from real quantum backends yielded worse results than noise-free simulations. However, the additional variation in the generated bit-vectors could also help to generate solutions of lower cost. This is observed in figure~\ref{fig:cdf_HW_128TRS}, where the hardware results yielded bit-vectors of lower cost than the lowest simulated vectors with a probability of more than 10\%. Noise does not necessarily move the distribution towards uniform random bit-vectors: On real hardware, the decay into the physical ground state is more likely than the excited state. Depending on the $\sigma_z$-to-bit mapping, this can result in a larger or smaller number of settled transactions than uniform randomness.

\smallskip

Figure~\ref{fig:ViolxTRS_HW_128TRS} emphasizes the need for classical post-processing methods that search for feasible solutions in the vicinity of infeasible solutions generated by the PQC (cf.~\ref{subsec:outlook}): None of the bit-vectors generated by both simulation and real hardware fulfil all the constraints on the security-account balances (cf. equation~\ref{eq:constraints}). Alternatively, the cost penalty $\lambda$ could be increased to put even higher priority on the balance constraints relative to the maximization of the number of transactions.



% \paragraph{Impact of noise} While to the most part, the noisy results obtained from real quantum hardware yield worse graphs than the noise-free simulation, the additional variation in the generated bit-vectors can also help to generate solutions of lower cost. This is particularly obvious in figure~\ref{fig:cdf_HW_128TRS}, whose simulated training run converged to a cost value around the top 5\% of the total range and shows little variation in the generated bit-vectors (nearly vertical cumulative distribution function). The hardware results on the other hand generate bit-vectors of lower cost than the lowest simulated vectors, with a probability of more than 10\%. While in this sense, some noise appears to help in generating better solution candidate, only to a limited extent if the noise-free simulation outperforms uniformly random sampling. We also note that \texttt{ionq\_aria} still outperforms \texttt{ibm\_hanoi} even in the regime of small cost values, despite the larger spread of the latter. Noise does not necessarily move the distribution towards uniform random bit-vectors: On real hardware, the decay into the physical ground state is more likely than the excited state. Depending on the $\sigma_z$-to-bit mapping, this can result in a larger or smaller number of settled transactions than uniform randomness.


% Adopting the view that variation around the generated solution helps, classical post-processing methods that search for solutions in the vicinity of the solutions generated by the PQC (cf.~\ref{subsec:outlook}) may be promising. The need for the latter is also reinforced by figure~\ref{fig:ViolxTRS_HW_128TRS}, which shows that among the bit-vectors generated by the PQC -- be it simulated or on real hardware -- no solution fulfills all constraints on the security-account balances (cf. equation~\ref{eq:constraints}). Alternatively, the cost penalty $\lambda$ could be increased to put even higher priority on the balance constraints relative to the maximization of the number of transactions.








\begin{figure} %TODO: Maybe redo with normalized cost
    \begin{subfigure}[t]{0.47\textwidth}
        \includegraphics[width =1.0\linewidth]{img/HW2_69_ecdf_costs.png}
        \caption{Register-preserving ansatz}
        \label{fig:cdf_reg-pres-HW}
    \end{subfigure}
    \begin{subfigure}[t]{0.47\textwidth}
        \includegraphics[width =1.0\linewidth]{img/HW2_68_ecdf_costs.png}
        \caption{Hardware-efficient ansatz}
        \label{fig:cdf_hwe-HW}
    \end{subfigure}
    \caption[Hardware results 16 Transactions]{\colorbox{lightgray!30!white}{16 Transactions, 10 parties, 6 qubits, $d=4$, DESC, $n_a = 4$, disjoint covering} | Empirical cumulative distribution function (cf.~figure~\ref{fig:cdf}%\textsuperscript{*}
    ) of cost (not normalized) over bit-vectors generated by a trained PQC. Executed on a simulator (Simulation), IBMQ quantum computer (\texttt{ibm\_geneva}) and IonQ quantum computer (\texttt{ionq\_harmony}). Uniformly random bit-vectors are shown by a grey line (Random). For each generator, $1000$ bit-vectors were drawn from $2.4 \times 10^4$ shots. Each subfigure corresponds to a single optimization run in which the PQC was optimized using gradient descent. Both runs produce narrow distributions around a fixed bit-vector, resulting in a steep curve (especially in the noise-free simulation). \\
    % \small\textsuperscript{*} Note how \emph{steep} the cumulative function is for the simulation. This is due to only considering a fixed chosen PQC as opposed to figure~\ref{fig:cdf} where we uniformly average over the PQCs resulting from different training runs and configurations. The PQC used here was trained with gradient descent, resulting in the convergence to a sparse solution (nearly) always outputting an identical bit-vector.
    }\label{fig:cdf_HW}    
    
\end{figure}

% TODO: Potentially redo and have cost not normalized
% 128 Transactions, benchmarking-H128TRS2023-05-04, Job-ID 56, 24000 shots for IBM and IonQ aria
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.52\textwidth}
        \includegraphics[width =1.0\linewidth]{img/HWibm_hanoi-ionq_aria_56_ecdf_n500.png}
        \caption{Empirical cumulative distribution function (cf. figure~\ref{fig:cdf}). To generate the blue dotted line, showing the distribution of uniformly random bit-vectors, we generated $10^6$ such vectors, the cost of which was used to normalize the x-axis.}
        \label{fig:cdf_HW_128TRS}
    \end{subfigure}
        \begin{subfigure}[t]{0.47\textwidth}
        \includegraphics[width =1.0\linewidth]{img/HWibm_hanoi-ionq_aria_56_Hist2D_n500_Securities_.png} 
        \caption{Scatter-plot of sampled bit-vectors. For overlaps, scatter-size scales with degeneracy. The x-axis shows the negative sum of final security-account balances over all parties with negative balances upon settlement according to the corresponding bit-vector. The number of transactions is the $L_1$ norm of the corresponding bit-vector. %The distribution-histograms are shown as marginal plots.
        }
        \label{fig:ViolxTRS_HW_128TRS}
    \end{subfigure}
    \caption[Hardware results 128 Transactions]{\colorbox{lightgray!30!white}{128 transactions, 41 parties, 19 qubits, hardware-efficient ansatz, $d=1$, DESC, $n_a = 16$, disjoint covering} | Visualization of results for 128 transactions on the \texttt{ibm\_hanoi} and \texttt{ionq\_aria} backends ($2.4 \times 10^4$ shots, 500 bit-vectors).}
    \label{fig:ionq_ibm_128trs_HW}
\end{figure}











==> 04_Conclusion.tex <==
Increasing the scope of tractable problems and benchmarking with industry data is important to gauge the applicability of heuristics-reliant variational quantum algorithms to optimization and to find promising applications. In this work, we extended the qubit-efficient encoding in~\cite{tan_qubit-efficient_2021} by providing explicit formulas of the cost objective and its gradient for arbitrary number of ancilla qubits. We introduced a new ansatz for uniform register sampling. We argue that register-preserving ansätze have the additional benefits of numerical stability, shot-reductions and selective sampling of individual registers, and expressing the cost estimator as a Hermitian observable.% (\ref{app:cost_as_observable}).

We demonstrate our methods on mixed binary optimization problems arising from financial transaction settlement ~\cite{braine_quantum_2019}, benchmarking problems of up to 128 transactions and 41 parties constructed from transaction data provided by a regulated financial exchange.
We also showed how the optimal slack variables can be obtained without the need for an outer loop optimization. We observed that our qubit-efficient methods outperformed standard QAOA, even when executed on quantum backends. Our proposed register-preserving ansatz stood out as best in many of the instances considered. 


% Increasing the scope of tractable problems and benchmarking with industry data is important to gauge the applicability of heuristics-reliant variational quantum algorithms to optimization and find promising applications.
% In this work, we took a step towards applying a quantum solver to problems of relevant size and generality, improving on and extending previous results (\cite{tan_qubit-efficient_2021, braine_quantum_2019}). 


% \subsection{Methods}

% We extended the qubit-efficient encoding in~\cite{tan_qubit-efficient_2021} by providing explicit formulas of the cost objective for arbitrary number of ancilla qubits and its gradient.
% This heuristic cost estimator~\ref{eq:cost_estimator} was proven (lemma~\ref{lemma:cost_estimator}) to be an unbiased estimate for the expected sampling cost (equation~\ref{eq:QUBO_as_expectation_min}) for greedy bit-vector sampling (algorithm~\ref{alg:greedy_sampling} in the appendix) and disjoint covering of the problem-variables through the qubit-efficient register-mapping $\mathcal{A}$.

% We furthermore propose to ensure uniform register sampling by either adding an additional regularization term equ.~\ref{eq:reg_pres_penalty} to the cost objective or by using a register-preserving ansatz. We introduce equivalent mathematical definitions of the latter, proving that every register-preserving unitary effectively corresponds to a basis-permutation on the register-qubits and arbitrary register-conditioned unitaries on the ancillas qubits (theorem~\ref{theorem:reg_preserving}). We argue that register-preserving ansätze have the additional benefit of incorporating symmetries, simplifying the cost estimator, allows for selective sampling of individual registers, and the expression of the cost estimator as a Hermitian observable (\ref{app:cost_as_observable}).


% Building on~\cite{braine_quantum_2019}, we demonstrate how to apply our qubit-efficient methods to the mixed binary optimization problem arising from financial transaction settlement. We contribute methods to reduce variance in the data (section~\ref{subsec:transaction_settlement_methods}) and substitute continuous slack variables in the optimization (equ.~\ref{eq:slack_estimator}). 

% Most of our methods are directly applicable beyond transaction settlement to any QUBO problem with linear inequality constraints, setting it apart from other qubit-efficient methods to the best of our knowledge.


% \subsection{Results}

% We construct benchmarking problems of up to 128 transactions and 41 parties by using transaction data provided by a regulated financial exchange, far exceeding the previous study by IBM and Barclays (\cite{braine_quantum_2019}), which only considered problems of at most 7 transactions.

% We demonstrate that our qubit-efficient methods slightly outperform standard QAOA, while reducing the number of qubits required at the cost of sampling overhead. Our proposed register-preserving ansatz stands out as performing best in many of the configurations considered. 
% Overall however, the performance differences between QAOA and our qubit-efficient methods, register-preserving and hardware-efficient circuits as well as between varying number of ancillas for encoding correlations, were rather minor, warranting further investigation.

% We run pre-trained quantum circuits on real hardware of IBM Quantum and IonQ, observing similar performance for a hardware-efficient circuit ansatz and significant advantages of IonQ for a register-preserving ansatz. The latter is most likely due to the all-to-all connectivity of trapped ion hardware, opposed to lattice connectivity on superconducting quantum computers. Real quantum backends saw both improvements over the noise-free simulation in the best 10\% of bit-vectors generated, as well as worse cost values for more than half the bit-vectors generated.

% We observed that our qubit-efficient methods slightly outperformed the standard QAOA while requiring fewer qubits but came with additional sampling overhead. 
% Our proposed register-preserving ansatz stood out as best in many of the instances considered, especially when executed noise-free or on the quantum backends offered by IonQ.


% While we show applicability to significantly larger transaction settlement problems than previous studies, our results also suggest caution as none of the methods benchmarked output constraint-satisfying bit-vectors at 128 transactions, despite achieving cost values in the best five percent. This study focused on increasing the size and generality of problems approachable by quantum methods. However, improving the solution quality is equally important for these methods to provide useful value on real problems.


% \subsection{Outlook and remaining open questions}
\label{subsec:outlook}



% To get a full picture of the potential of our methods to deliver real business value and potential advantages over classical methods, a comparison to state-of-the-art classical solvers on problem instances faced in real scenarios is needed. Suitable problem instances can -- due to the generic formulation as a QUBO problem with linear inequality constraints -- be beyond financial transaction settlement.\footnote{For a list of examples see~\cite{punnen_quadratic_2022} ch.~2.2(.1).} 


\paragraph{Post-processing} 
While not explored in this work, post-processing by projecting sampled solutions to valid bit-vectors fulfilling all problem constraints%, similar to the methods proposed in \cite{goh_techniques_2022}, 
may be a necessity. One possible method to do so includes projecting a solution bit-vector generated by the QS to the best bit-vector \emph{in the vicinity} that fulfils all constraints. Restricting the search to a ball of Hamming distance $\leq k$, solutions can be sampled at the asymptotic runtime of $O(I^k)$ (as opposed to $2^I$ for a full search). While without guarantees for the optimality or even existence of a close valid solution, one may hope that if the QS provides solutions of high quality, only small adjustments are needed to obtain a good solution which adheres to all constraints. This search can be refined with heuristics, e.g.~by only adjusting transactions involving parties (and potentially their k-nearest-neighbours on the graph) whose balance constraints are violated.


% For this purpose, post-processing by projecting sampled solutions to valid bit-vectors fulfilling all problem constraints may well be a necessity. The constraints may be enforced by projecting a solution bit-vector generated by the QS to the best bit-vector \emph{in the vicinity} that fulfils all constraints. What counts as vicinity is partly set by computational limitations. While without guarantees for the optimality or even existence of a close valid solution, one may hope that if the QS provides solutions of high quality, only small adjustments are needed to obtain a good solution which adheres to all constraints. Restricting the search to a ball of Hamming distance $\leq k$, solutions can be sampled by flipping $n \in \{1,\ldots, k\}$ bits at the asymptotic runtime of $O(I^k)$ (as opposed to $2^I$ for a full search).

% An alternative to brute force proximity search is to design heuristic projections. For the example of our balance constraints in equ.~\ref{eq:constraints}, a heuristic projection may only adjust transactions involving parties (and potentially their k-nearest-neighbours) whose balance constraints are violated.
% Even more narrow, one could invalidate outgoing transactions of the appropriate security for parties whose constraints are violated until these parties end on non-negative balances. 

% For the purpose of this proof of concept we did not implement any such projection, for a related example (with a different set of constraints) we refer to~\cite{goh_techniques_2022}.


\paragraph{Method exploration} 
Overall, further exploration of different ancilla-register-mappings, variational (register-preserving) ansätze, optimization algorithms and (scaling of) meta-parameters such as circuit depth, penalty terms and step-size is warranted to validate and refine the qubit-compression approach presented in this work. 
For example, how the restrictions given by theorem~\ref{theorem:reg_preserving} regarding the register-preserving ansatz can best be extended in practice, e.g. by changing the computational basis and keeping track of phases on the ancilla qubits (cf.~\ref{lemma:reg_pres_sometimes}), is still an open question. 
Another important consideration is the lack of correlation between the individual measurements in the sampling algorithm used in this work. Exploring sample rejection or the addition of hidden layers to the ansatz provides one avenue to extend the probability distributions of $\myvec x$ which our PQC parameterizes. 

% Overall, further experimental exploration of different ancilla-register-mappings, variational (register-preserving) ansätze, optimization algorithms and (scaling of) meta-parameters such as circuit depth, penalty terms and step-size is warranted to validate and refine the qubit-compression approach presented in this work. Table~\ref{tab:parameters_explored} gives a comprehensive overview of different design considerations for the application of the qubit-efficient encoding and the variations explored in this work, as well as some directions that could be further explored.

% Mapping techniques from register-qubits to subsets $A_r\in \mathcal{A}$ of the problem variables and the sampling of solutions from a qubit-efficient PQC can take inspiration from existing work on divide-and-conquer approaches. In doing so, one needs to keep in mind that changing the algorithm for sampling bit-vectors potentially implies changes to the form of the cost estimator. One important limitation of the sampling algorithm (algorithm~\ref{alg:greedy_sampling}) used in this work, is the lack of correlation between individual measurements. Exploring sample rejection or the addition of hidden layers to the ansatz provides one avenue to extend the probability distributions of $\myvec x$ which our PQC parameterizes.

% Improving both the variational ansatz as well the classical optimization is important to avoid the many pitfalls plaguing VQAs, such as bad local minima, barren plateaus, noise, sampling overhead and lack of theoretical guarantees. %TODO: Maybe some references
% For the ansatz, register-preserving ansätze provide a promising avenue to further explore due various theoretical (end of section~\ref{subsec:vqa_ansatz}) and benchmarked (section~\ref{sec:results}) advantages. An interesting open question is, whether the restrictions given by theorem~\ref{theorem:reg_preserving} can be expanded in practice (cf.~\ref{lemma:reg_pres_sometimes}, changing the computational basis, keeping track of phases on the ancilla qubits $\ldots$).

\medskip

Our methods, despite being tested on synthetic problems, demonstrated the broad applicability of quantum algorithms beyond small toy examples. Witnessing advantages of our methods over classical solvers would require a comparison to state-of-the-art classical solvers on problem instances faced in real scenarios. 
Most of our methods are directly applicable beyond the transaction settlement problem to any QUBO problem with linear inequality constraints, setting them apart from other qubit-efficient methods to the best of our knowledge and making them suitable to tasks beyond settling financial transactions.\footnote{For a list of examples see~\cite{punnen_quadratic_2022} ch.~2.2(.1).} 



% \begin{table}[t]
% \centering
% \begin{tabular}{@{}l c c@{}}
% \emph{Design consideration} & \emph{Explored in this work} & \emph{Outlook / references} \\ \cmidrule{1-3}
% \textbf{Pre-processing} & & \\
% \quad Pre-fixing QUBO variables& {\large-} & \cite{glover_logical_2018, lewis_quadratic_2017}\\
% \quad Data scaling & Balance re-scaling per party (\ref{subsec:transaction_settlement_methods})& Different scaling factor\\
% \textbf{Optimizer architecture} &&\\
% \quad Sampling algorithm & 
% \begin{tabular}{@{}c@{}}Greedy sampling (alg.~\ref{alg:greedy_sampling}), \\ Rejection sampling$^*$, Hidden layer$^*$ (\ref{app:sampling})\end{tabular} & \multirow{2}{*}{
% \begin{tabular}{@{}c@{}}Methods from divide \& conquer \\ approaches (\cite{harrigan_quantum_2021, otterbach_unsupervised_2017, pelofske_quantum_nodate, shaydulin_qaoa_2023, zhu_multi-round_2022, fujii_deep_2022})
% \end{tabular}}\\
% \quad Register-mapping & k-means$^*$ & \\
% \quad Cost objective & \begin{tabular}{@{}c@{}}Heuristic, Balance-constraints and \\ register-uniformity as penalty (\ref{subsec:cost}), \\ $\langle H \rangle^*$ (\ref{app:cost_as_observable}) \end{tabular}& \begin{tabular}{@{}c@{}}Adapt heuristic to sampling algorithm, \\derive for redundant covering, \\classical shadows (\cite{huang_predicting_2020})\end{tabular}\\ 
% \quad Variational ansatz &  Hardware-efficient, Register-preserving &
% \begin{tabular}{@{}c@{}} Exploration register-preserving,\\ viable remedy for barren plateaus?\end{tabular}\\
% \textbf{Optimization} && \\
% \quad Parameter initialization & Uniform random $\in [0,2\pi]$ & \cite{egger_warm-starting_2021, akshay_parameter_2021, grant_initialization_2019, mitarai_generalization_2019, truger_warm-starting_2023, egger_warm-starting_2021}\\
% \quad Optimization step & 
% \begin{tabular}{@{}c@{}}COBYLA, Gradient descent (\ref{subsec:opt}), \\ slack variable substitution (\ref{subsec:cost}) 
% \end{tabular}& \cite{barkoutsos_improving_2020, schuld_evaluating_2019, ostaszewski_structure_2021, nakanishi_sequential_2020, skolik_layerwise_2021, bharti_noisy_2022}\\
% \quad Convergence criteria & Limit on steps & \\
% \quad Meta-parameters &
% \begin{tabular}{@{}c@{}}
% $\lambda \in \{10, 10^2\},~\eta = 10^3$ 
%  $,~n_{\text{shots}}\in \{10^4, 2\times10^4\}$,\\
% $n_a \in \{1,2,4,8,16\}$, redundancy in covering,\\
% depth $d\in\{1,2,4,8\}$, step-size \ldots (\ref{subsec:qubit_compression}, \ref{subsec:cost})
% \end{tabular}
% & Adaptive choice \\
% \textbf{Post-processing} & & \\
% \quad Projection & Neighbourhood-search and heuristics$^*$ (\ref{subsec:outlook}) & \\

% \end{tabular}
% \caption{Overview of different design considerations when applying the qubit-efficient encoding to real optimization instances. The middle column gives a summary of the approaches explored in this work. The right column provides starting points for further exploration or references that could be adapted.\\
% $^*$only cursory exploration in this work}
% \label{tab:parameters_explored}
% \end{table}

==> tikz_ansatz.tex <==



%TODO: Maybe nicer drawing (vgl. Ben's paper)
\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.7\textwidth}
    \resizebox{\textwidth}{!}{
        \begin{quantikz}
        \lstick[wires=2]{Ancilla} 
            & \gate[wires=1]{R_Y(\theta_1)} \gategroup[wires=5,steps=5,style={dotted, cap=round, inner sep=7pt}]{Conditional rotations} &\qw ~...~ &\gate[wires=1]{R_y(\theta_{n_r})} & \qw &\qw &\qw &\qw \gategroup[wires=5,steps=3,style={dotted, cap=round, inner sep=7pt}]{Basis permutation} & \qw & \qw \\
            &\qw   &\qw &\qw &\qw & \gate[wires=1]{R_y(\theta_{n_r+1})} &\qw ~...~ & \qw & \qw&\qw\\
        \lstick[wires=3]{Register} 
            & \ctrl{-2} &\qw &\qw&\qw &\ctrl{-1} & \qw &\qw &\qw &\targ{}\\
            ~~~\raisebox{0.2cm}{\vdots} & & \qw ~...~  & \qw & \qw & \qw & \qw ~...~ & \targ{} & \qw ~...~ &\ctrl{-1}\\
            & \qw& \qw & \ctrl{-4} &\qw & \qw & \qw ~...~ & \ctrl{-1} & \qw &\qw
        \end{quantikz} 
    }
    \caption{Register-preserving ansatz}
    \label{fig:reg-pres_ansatz}
    \end{subfigure}
    \begin{subfigure}[t]{0.27\textwidth}
    \resizebox{\textwidth}{!}{
        \begin{quantikz}
        \lstick[wires=2]{Ancilla} 
            & \gate[wires=1]{R_Y(\theta_{1~})} \gategroup[wires=5,steps=1,style={dotted, cap=round, inner sep=7pt}]{Rotations} & \qw & \gategroup[wires=5,steps=2,style={dotted, cap=round, inner sep=7pt}]{Entangling} \qw & \targ{}\\
            &\gate[wires=1, ]{R_y(\theta_{n_a})} &\qw & \targ{} & \ctrl{-1}\\
        \lstick[wires=3]{Register} 
            &  ~~~\raisebox{0.2cm}{\vdots}~~~ & \qw & \ctrl{-1} & \targ{}\\
            & ~~~\raisebox{0.2cm}{\vdots}~~~ & \qw & \targ{} & \ctrl{-1}\\
            & \gate[wires=1]{R_y(\theta_{n_q})} & \qw & \ctrl{-1} & \qw
        \end{quantikz} 
    }
    \caption{Hardware-efficient ansatz}
    \label{fig:hwe_ansatz}
    \end{subfigure}
    \caption[Variational Ansatz]{One layer of the register-preserving ansatz (left) and the hardware-efficient ansatz (right) used in the result section. To obtain the PQC $U(\myvec \theta)$, these circuit layers $L$ are preceded by a Hadamard gate on every qubit and are repeated a chosen number $d$ of times (\emph{depth}), i.e. $U(\myvec \theta) = L(\myvec \theta)^d H^{\otimes n_q}$. Furthermore, in the case of the register-preserving ansatz, parameterized single-qubit $R_Y$ rotations were applied to all ancillas prior to the first layer.}
    \label{fig:var_ansatz}
\end{figure}
